Distributed Online Convex Optimization with Improved Dynamic Regret

In this paper, we consider the problem of distributed online convex optimization, where a group of agents collaborate to track the global minimizers of a sum of time-varying objective functions in an online manner. Specifically, we propose a novel distributed online gradient descent algorithm that relies on an online adaptation of the gradient tracking technique used in static optimization. We show that the dynamic regret bound of this algorithm has no explicit dependence on the time horizon and, therefore, can be tighter than existing bounds especially for problems with long horizons. Our bound depends on a new regularity measure that quantifies the total change in the gradients at the optimal points at each time instant. Furthermore, when the optimizer is approximatly subject to linear dynamics, we show that the dynamic regret bound can be further tightened by replacing the regularity measure that captures the path length of the optimizer with the accumulated prediction errors, which can be much lower in this special case. We present numerical experiments to corroborate our theoretical results.

==> tex/Experiements_bkup.tex <==
In this section, we investigate the performance of our proposed algorithm with numerical experiments based on a target tracking example. Specifically, we consider a sensor network consisting of $n=6$ nodes that collaboratively track $3$ time-varying signals of sinusoidal shape. Each signal $x_{j,t}^\ast$ can be written following form

\begin{equation*}
	\label{eqn:SinusoidalSignal}
	x_{j,t}^\ast = \begin{bmatrix}
	p_{j,t} \\ \dot{p}_{j,t}
	\end{bmatrix} = 
	\begin{bmatrix}
	A_j \sin(\omega_{j} t + \phi_j) \\ \omega_j A_j \cos (\omega_{j}t + \phi_j)
	\end{bmatrix},
\end{equation*}
where $p_{j,t}$ is the position, $\dot{p}_{j,t}$ is the velocity of target $j$, $A_j$ is the amplitude, $\omega_j$ is the angular frequency, and $\phi_j$ is the phase of the signal. Each signal is subject to an ODE with noise

\begin{equation}
	\label{eqn:SinusoidalODE}
	\dot{x}_{j,t}^\ast = \begin{bmatrix}
	0 & 1 \\ -\omega_{j}^2 & 0
	\end{bmatrix} x_{j,t}^\ast + w_{j,t},
\end{equation}
where $w_j$ is a zero mean Gaussian noise. The matrix governing the dynamical system in this example can be estimated by discretizing the solution of the ODE \eqref{eqn:SinusoidalODE}. In the simulation, the amplitudes $\{A_j\}$ and inital phases are uniformly generated from the intervals $[0, 2]$ and $[0, \pi]$, respectively. The doubly stochastic matrix $W$ used in step \eqref{eq:Algorithm_step1} is randomly generated and $\sigma_W = 0.8554$. The sampling frequency is set to $100$Hz. The measurement model of sensor $i$ at time $t$ is

\begin{equation}
	\label{eqn:Measurement}
	y_{i,t} = C_{i} x_{t}^\ast,
\end{equation}
where $x_t^\ast = [\dots; x_{j,t}^\ast; \dots]$ is the true target state, $y_{i,t} \in \mathbb{R} $ is the observation at sensor $i$, and $C_i \in \mathbb{R}^{1 \times 6}$ is the measurement matrix that is randomly generated. At time $t$, the global problem is defined as

\begin{equation}
	\label{eqn:GlobalSensing}
	\min_{x_t} \frac{1}{2} \sum_{i = 1}^{6} |C_{i}x_t - y_{i,t}|^2 \triangleq \frac{1}{2} \|Cx_t - y_t\|^2,
\end{equation}
where the matrix $C$ and the vector $y_t$ stack all measurement matrices $C_i$ and local measurements $y_{i,t}$. We assume that $C^{T}C$ is positive definite in order to guarantee that the objective is strongly convex. This guarantees that the target state $x_t$ is determined uniquely given all local observations at time $t$. 
%In this example, the gradient path-length regularity $\mathcal{V}_T = 0$. To see this, we have that $\nabla f_{i,t}(x_t^\ast) = C_i^T (C_ix_t^\ast - y_{i,t}) = 0$ at every $t$.
\begin{figure}
	\centering
	\subfigure[Periodicity $1000$s]{\includegraphics[width=.88\columnwidth]{figure/tracking_theoreticalStepsize_1000s.eps}}
	\subfigure[Periodicity $10$s]{\includegraphics[width=.88\columnwidth]{figure/tracking_theoreticalStepsize_10s.eps}}	
	\caption{Tracking performance of Algorithm~\ref{alg:oco_nprediction} with theoretical stepsize bound in Theorem~\ref{thm:BoundRegret}}
	\label{fig:tracking_theoreticalStepsize}
\end{figure}

\subsection{Choice of stepsize}
In this section, we track signals defined as in \eqref{eqn:SinusoidalODE} with periodicity $1000$s and $10$s using Algorithm~\ref{alg:oco_nprediction} and assuming that $A$ is the identity matrix, i.e. we do not take any predictability of the future into account. In both experiments, we let the step size $\alpha = 2.45 \times 10^{-5}$ in accordance with the assumptions of Theorem~\ref{thm:BoundRegret}. The tracking performance is shown in Figure~\ref{fig:tracking_theoreticalStepsize}. We observe that using this theoretical stepsize, Algorithm~\ref{alg:oco_nprediction} performs better in tracking signals with periodicity $1000$s than $10$s. 
This is unsurprising; the motion of the targets is sampled more frequently when the periodicity is 1000s.
In particular, the theoretical step size $\alpha$ is too conservative, preventing our algorithm from tracking quickly moving targets. However, we can use larger stepsizes than the theoretical ones given in Theorem~\ref{thm:BoundRegret} and achieve better performance. Specifically, in Figure~\ref{fig:tracking_EmpStep} (a), we observe that for a more aggressive selection of the stepsize, the accumulated regret becomes smaller, implying better tracking performance. And in Figure~\ref{fig:tracking_EmpStep} (b), we show that the tracking performance of Algorithm~\ref{alg:oco_nprediction} for the target signal of periodicity $10$s can be improved using $\alpha = \frac{1}{2L_g} \approx 0.2$.
\begin{figure}
	\centering
	\subfigure[Regret under different stepsizes]{\includegraphics[width=.9\columnwidth]{figure/trackingRegret_EmpStep.eps}}
	\subfigure[Tracking performance when $\alpha = \frac{1}{2L_g}$]{\includegraphics[width=.9\columnwidth]{figure/tracking_EmpStep.eps}}	
	\caption{Tracking performance of Algorithm~\ref{alg:oco_nprediction} with empirical stepsizes $\alpha = [\frac{1}{2L_g}, \frac{1}{10L_g}, \frac{1}{100L_g}, \frac{1}{1000L_g}]$ and target signals are of periodicity $10$s.}
	\label{fig:tracking_EmpStep}
\end{figure}

%{\color{red} Fix the simulation. Put the noise in the measurement model instead of dynamics model. Try different sampling frequency and noise.}

\subsection{Effect of prediction}
We also investigated the role of the prediction step in the empirical performance of Algorithm~\ref{alg:oco_nprediction} by comparing numerical prediction of the dynamical system based on discretization as mentioned above to the case without prediction, i.e. where $A$ in ~\eqref{eq:Algorithm_step2} is the identity matrix. The comparison was conducted by tracking targets of periodicity $10s$ with stepsize $\alpha = \frac{1}{2L_g}$. The tracking performance and dynamic regret are presented in Figure~\ref{fig:tracking_WtPredict}. In Figure~\ref{fig:tracking_WtPredict}(a), we observe that Algorithm~\ref{alg:oco_nprediction} that incorporating numerical prediction can greatly improve the dynamic regret of an algorithm compared to not incorporating any prediction (note that the figure is in log-scale), though note that the shape of both cumulative regret curves are roughly the same. This improvement is further corroborated in Figures~\ref{fig:tracking_WtPredict} (b) and (c); the dashed curves indicating the actual optimal points are generally overlapped by the solid curves of the estimated positions when prediction is utilized, whereas there is little overlap if no prediction is used.
%{\color{blue}
%This is because the regularity term $\mathcal{P}_T^A$ in \eqref{eqn:PathLength} accumulates the prediction error $\|x_{t+1}^\ast - Ax_t^\ast\|$ when prediction is used rather than the path length of the optimizers $\|x_{t+1}^\ast - x_t^\ast\|$ when no preciction is applied. When the prediction error $\|x_{t+1}^\ast - Ax_t^\ast\|$ is small, the accumulated prediction error $\sum_{t=0}^{T-1} \|x_{t+1}^\ast - Ax_t^\ast\|$  can be much smaller than the path length of the optimizers $\sum_{t=0}^{T-1}\|x_{t+1}^\ast - x_t^\ast\|$.}

\subsection{Comparison with existing algorithms}
We now compare the performance Algorithm~\ref{alg:oco_nprediction} to the online distributed gradient (ODG) algorithm studied in \cite{shahrampour2018distributed}. Both algorithms are implemented with prediction. The regrets achieved by these algorithms under different stepsizes are presented in Figure~\ref{fig:Compare2Ali}. Though both algorithms have comparable performance for the smaller step sizes, the behavior is wildly different for the larger step sizes. While ODG diverges for stepsizes $\frac{1}{L_g}$ and $\frac{2}{L_g}$, Algorithm~\ref{alg:oco_nprediction} is stable using these stepsizes and, consistent with previous observations, the cumulative regret with these stepsizes is smaller than the previous stepsizes for which both algorithms successfully converged. This behavior was also observed in multiple other randomly generated examples, and is consistent with that observed in \cite{ZhangCDC2019_OnlineOptimization}.

\begin{figure}
	\centering
	\subfigure[Regret of Algorithm~\ref{alg:oco_nprediction} with or without prediction]{\includegraphics[width=.9\columnwidth]{figure/trackingRegret_WtPredict.eps}}
	\subfigure[Tracking performance without prediction]{\includegraphics[width=.45\columnwidth]{figure/tracking_NoPredict.eps}}
	\subfigure[Tracking performance with prediction]{\includegraphics[width=.45\columnwidth]{figure/tracking_WtPredict.eps}}				
	\caption{Comparison of regret and tracking performance of Algorithm~\ref{alg:oco_nprediction} with and without prediction, stepsizes $\alpha = \frac{1}{2L_g}$ and target signals are of periodicity $10$s.}
	\label{fig:tracking_WtPredict}
\end{figure}

\subsection{Necessity of the gradient path-length regularity}
Since the regret bound in \cite{shahrampour2018distributed} is only related to the optimizer path-length regularity term $\mathcal{P}_T^A$, it is natural to ask whether the dependence of the theoretical regret bound of Algorithm~\ref{alg:oco_nprediction} on $\mathcal{V}_{T}$ can be removed. In the following, we empirically show that the regret bound $R_T^d$ of using Algorithm~\ref{alg:oco_nprediction} not only depends on $\mathcal{P}_T^A$ in general, but also on $\mathcal{V}_{T}.$ To do this, we construct a numerical example for which $\mathcal{P}_T^A = 0$ for all $T$ but $R_T^d$ grows at the same speed as the regularity term $\mathcal{V}_T$. 

Consider the distributed estimation problem shown in Figure~\ref{fig:RotatingRods}, where two targets are moving along circular paths around the origin. Let $\theta_1(t)$ and $\theta_2(t)$ denote their angles from the horizontal axis, and let $R_{1}$ and $R_{2}$ denote the distances of the targets with from the origin. Four sensors need to estimate these distances, though each sensor can only measure the projected coordinate of one target onto one axis. Letting $y_t$ denote the collected measurement at time $t,$ we assume the $y_{t}$ received are of the following form

\begin{equation}
\label{eqn:MeasurementModel}
\begin{split}
y_t &= \begin{bmatrix}
\cos \theta_1(t) & 0 \\ \cos \theta_2(t) & 0 \\ 0 & \sin \theta_1(t) \\ 0 & \sin \theta_2(t)
\end{bmatrix}
\begin{bmatrix}
R_1 \\ R_2
\end{bmatrix} + v_t \\
&= C_t \; \begin{bmatrix}
R_1 \\ R_2
\end{bmatrix} + v_t,
\end{split}
\end{equation}
where each entry of $y_t$ signifies one sensor's measurement and $v_t$ is a noise term at time $t$ to be specified.
\begin{figure}[t]
	\centering
	\includegraphics[width=.9\columnwidth]{figure/trackingRegret_Compare2Ali.eps}
	\caption{Comparison of the regrets between Algorithm~\ref{alg:oco_nprediction} (solid lines) and the online distributed gradient algorithm in \cite{shahrampour2018distributed} (dashed lines). Both algorithms are run with stepsizes $\alpha = [\frac{2}{Lg}, \frac{1}{Lg}, \frac{1}{2Lg}, \frac{1}{10Lg}]$.}
	\label{fig:Compare2Ali}
\end{figure}
We assume that $R_1$ and $R_2$ are constant, so that the matrix governing the dynamical system in Assumption~\ref{assum:DynamicalMatrix} is the identity matrix. We also assume that the four sensors are connected in a cyclic graph. We wish to investigate the performance of Algorithm~\ref{alg:oco_nprediction} in tracking the optimizer of the global estimation problem

\begin{equation}
\label{eqn:GlobalProblem}
\min_{x_t} \; f_t(x_t) := \frac{1}{2} \sum_{i=1}^{4} \| [C_t]_i x_t - [y_t]_i \|^2
\end{equation}
\noindent where $[C_t]_i$ denotes the $i$th row of the matrix $C_t$.

We specifically design the noise terms $v_t$ in the measurement model \eqref{eqn:MeasurementModel} so that the optimizer $x_t^\ast$ of the objective is constant for all $t$, which implies that $\mathcal{P}_{T}^{A} = 0.$ To achieve this, observe that we can write the first order optimality condition as

\begin{equation}
\label{eqn:FirstOrderOptimality}
\nabla f_t(x_t) |_{x_t = x_t^\ast} = C_t^T (C_t x_t^\ast - y_t) = 0.
\end{equation}
Replacing $y_t$ in \eqref{eqn:FirstOrderOptimality} with \eqref{eqn:MeasurementModel}, we have that

\begin{equation}
\label{eqn:Derivation_1}
C_t^T(C_t x_t^\ast - C_t \begin{bmatrix}
R_1 \\ R_2
\end{bmatrix} - v_t) = 0.
\end{equation}
Thus, to ensure that $x_t^\ast = [R_1, R_2]^T$ for all $t,$ we see that $v_t$ must lie in the kernel of the matrix $C_t^T$. 

In our simulation, we let the vector $v_t$ be a unit vector in the kernel space of $C_t^T$, guaranteeing that $x_t^\ast = [R_1, R_2]^T$ for every $t$ and $\mathcal{P}_T^{A} = 0$ for all $T$ as mentioned above. However, the regularity term $\mathcal{V}_T^A$ is nonzero and grows with time because 

$$\nabla f_{i,t}(x_t^\ast) = [C_t]_i^T([C_t]_ix_t^\ast - [y_t]_i) = [v_t]_i [C_t]_i^T$$ so 

\begin{align*}
&\|g_{t+1}(Ax_{t}^\ast) - g_{t}(x_{t}^\ast)\| \\
&= \sum_{i=1}^{4}\|[v_{t+1}]_i [C_{t+1}]_i^T - [v_t]_i [C_t]_i^T\|^2 > 0
\end{align*} 
for all $t$. 

\begin{figure}[t]
	\centering
	\includegraphics[width=.6\columnwidth]{figure/example.pdf} %FIG_ReschuArchitecture2
	\caption{Estimation of the lengths of two rotating rods}
	\label{fig:RotatingRods}
\end{figure}

We run both Algorithm~\ref{alg:oco_nprediction} and ODG to track the optimizer of problem~\eqref{eqn:GlobalProblem} for $T = 1\times10^4$ time steps. The regret curves together with the regularity curve of $\mathcal{V}_T$ are shown in Figure~\ref{fig:Regret_Regularity}. It is clear that the regret $R_d^T$ grows with the same rate as the regularity term $\mathcal{V}_T$. Similar behavior was noticed when increasing $T$ to $1 \times 10^6.$ This is because of the gradient estimator $y_{i,t}$ in \eqref{eq:Algorithm_step3} in Algorithm~\ref{alg:oco_nprediction}. Each local $y_{i, t}$ estimates the summation of the local gradients $\sum_i \nabla f_{i,t}(x_{i,t})$. However, even when this term equals 0,  if $ \nabla f_{i, t+1}(x_{i,t+1}) - \nabla f_{i, t}(x_{i,t}) \neq 0$ for all $t$, the consensus estimator $y_{i,t}$ is continuously perturbed away from the correct estimate. This perturbation error is accumulated in the regret through the gradient update in \eqref{eq:Algorithm_step1}. 

It is interesting to note that even though ODG does not apply the gradient estimator $y_{i,t}$ in Algorithm~\ref{alg:oco_nprediction}, it also suffers from such perturbations as shown in Figure~\ref{fig:Regret_Regularity}. It is most likely that the error from the perturbations is accumulated directly in the local gradient calculation, though we will not investigate this further and will leave this for future work.

\begin{figure}[t]
	\centering
	\includegraphics[width = 0.9\columnwidth]{figure/Regret_Regularity}
	\caption{The accumulation of the regret $R_d^T$ (green line) and the gradient path-length regularity $\mathcal{V}_T$ (red line) by running Algorithm~\ref{alg:oco_nprediction} to solve problem~\eqref{eqn:GlobalProblem}.}
	\label{fig:Regret_Regularity}	
\end{figure}

